AJAHR: Amputated Joint Aware 3D Human Mesh Recovery

Existing human mesh recovery methods assume a standard human body structure, overlooking diverse anatomical conditions such as limb loss. This assumption introduces bias when applied to individuals with amputations - a limitation further exacerbated by the scarcity of suitable datasets. To address this gap, we propose Amputated Joint Aware 3D Human Mesh Recovery (AJAHR), which is an adaptive pose estimation framework that improves mesh reconstruction for individuals with limb loss. Our model integrates a body-part amputation classifier, jointly trained with the mesh recovery network, to detect potential amputations. We also introduce Amputee 3D (A3D), which is a synthetic dataset offering a wide range of amputee poses for robust training. While maintaining competitive performance on non-amputees, our approach achieves state-of-the-art results for amputated individuals. Additional materials can be found at the project webpage.

==> equtations/BPAC_Loss.tex <==
% \begin{equation} \label{eq:bpac_loss}
% \begin{gathered}
% \mathcal{L}_{cls} = \sum_{p \in \mathrm{{L\_{arm}, R\_{arm}, L\_{leg}, R\_{leg} \}}}} CE(h_p, lb),
% \end{gathered}
% \end{equation}
\begin{equation} \label{eq:bpac_loss}
\mathcal{L}_{cls} = \sum_{p \in \{L\_{arm}, R\_{arm}, L\_{leg}, R\_{leg}\}} CE(h_p, lb),
\end{equation}




==> equtations/BPAC_head.tex <==
\begin{equation} \label{eq:codebook_mapping}
\begin{gathered}
h_p = \mathcal{H}_p(F_{amp}, F_{non\_amp}),  \\
h_{token} = \mathcal{H}_{token}(F_{amp}, F_{non\_amp}).
% \mathrm{h_{L\_arm}}, \mathrm{h_{R\_arm}}, \mathrm{h_{L\_leg}}, \mathrm{h_{R\_leg}}
\end{gathered}
\end{equation}
where $h_{p} \in \mathbb{R}^{d_p},~~ h_{token} \in \mathbb{R}^{d_{token}}$.


==> equtations/BPAC_head2.tex <==
\begin{equation} \label{eq:codebook_mapping}
\begin{gathered}
\mathrm{h_{L_{arm}}},\mathrm{h_{R_{arm}}}\mathrm{h_{L_{leg}}},\mathrm{h_{R_{leg}}\in\mathbb{R}^{d_p}},~~ h_{token}\in\mathbb{R}^{token}.
\end{gathered}
\end{equation}


==> equtations/BPAC_input.tex <==
\begin{equation} \label{eq:codebook_mapping}
\begin{gathered}
F = \Phi(\mathrm{X}).
\end{gathered}
\end{equation}


==> equtations/Rotation_to_6D.tex <==
\begin{equation} \label{eq:theta_transformation}
\begin{gathered}
    \theta_i \in \mathbb{R}^{3 \times 3}
    \;\;\overset{\text{6D}}{\longmapsto}\;\;
    \theta_i 
    = \smash{\begin{bmatrix}
        \theta_i^{(1)}, \theta_i^{(2)}
      \end{bmatrix}^{T}} \in \mathbb{R}^{6}, \\
    \quad \text{where } \theta_i^{(1)}, \theta_i^{(2)} \in \mathbb{R}^{3},
    \quad i = 1, 2, \dots, 21.
\end{gathered}
\end{equation}


==> equtations/Tokenizer_loss.tex <==
\begin{equation}\label{eq:tokenizer_loss}
\begin{gathered}
\mathcal{L}_{total} = \lambda_{mix} \mathcal{L}_{mix} + \lambda_{cb} \mathcal{L}_{cb} + \lambda_{commit} \mathcal{L}_{commit} \\
= \lambda_{mix} \mathcal{L}_{mix} + \lambda_{cb} \lVert sg(z) - e \rVert_2 + \lambda_{commit} \lVert z - sg(e) \rVert_2.
\end{gathered}
\end{equation}


% \vspace{-10pt}
% \begin{equation} \label{eq:tokenizer_loss}
% \begin{gathered}
% \mathcal{L}_{total} = \lambda_{mix}\mathcal{L}_{mix} + \lambda_{cb}\mathcal{L}_{cb} + \lambda_{commit}\mathcal{L}_{commit} \\ = \lambda_{mix}\mathcal{L}_{mix} + \lambda_{cb}||sg(z)-e||_2 + \lambda_{commit}||z-sg(e)||_2.
% \end{gathered}
% \end{equation}


==> equtations/arch1.tex <==
\begin{equation} \label{eq:arch1}
\begin{gathered}
\mathbf{\hat{y}_p} =
\begin{cases}
0, & \text{if } \arg\max (h_p) = lb_{non\_amp} \\
1, & \text{otherwise.}
\end{cases}
\end{gathered}
\end{equation}



==> equtations/arch2.tex <==
\vspace{-10pt}
\begin{equation} \label{eq:arch}
\begin{gathered}
\hat{\theta} =
\begin{cases} 
\sigma{(\mathcal{T})}\times\mathbf{C}_{amp} & \text{if } max(\mathbf{\hat{y})}\ = 1 \\
\sigma{(\mathcal{T})}\times\mathbf{C}_{non\_amp} & \text{otherwise}
\end{cases}
\end{gathered}
\end{equation}


==> equtations/codebook_mapping.tex <==
\begin{equation}
\begin{gathered}
    \hat{z}_i = \arg\min_{e_i \in \mathbf{C}} \| z_i - \epsilon_i \|_2\end{gathered}.
    \label{eq:codebook_mapping}
\end{equation}

==> equtations/mix_loss.tex <==
\vspace{-6mm}
\begin{equation} \label{eq:tokenizer_loss}
\begin{gathered}
\mathcal{L}_{mix} = \mathcal{L}_{2}(\theta - \hat{\theta}) + \mathcal{L}_{2}(J_{3D} - \hat{J}_{3D}) + \mathcal{L}_{2}(V - \hat{V}).
\end{gathered}
\end{equation}

==> suppl_tex/datasynthesis.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{fig/datasynthesis.pdf}
\vspace{-0.2cm}
\caption{\textbf{Pipeline for Synthesizing Images of Individuals with Amputations.} The input image (\(I_{\mathit{in}}\)) is sourced from benchmark datasets~\cite{h36m_pami, mpii, mscoco} and processed through ScoreHMR~\cite{scorehmr}, an HMR-based model (*), which infers SMPL parameters from the image.  We extracted the human region using SAM (Segment Anything Model)~\cite{SAM} for masking and then removed the region using LaMa~\cite{lama} to generate the background. Finally, the generated human mesh was projected onto the background image to create the final image($I_{\mathit{out}}$).}
\label{fig:pipe_line}
\end{figure*}

==> suppl_tex/zeropose.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{fig/rebuttal/rebuttal_zero_pose.pdf}
\caption{\textbf{Effect of varying the pose parameters on the left wrist from $-1.0$ to $1.0$.}}
\label{fig:zeropose}
\end{figure}


==> table/AMPUTATION_DATASET_TABLE.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{A3D} & \multicolumn{3}{c}{ITW-amputee} \\ 
\cline{2-7}
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
\hline
HMR2.0~\cite{4dhumans}       & 89.35 & 96.75 & 86.14 & \textbf{110.33} & 154.43 & 121.83 \\
BEDLAM-CLIFF~\cite{bedlam, cliff} & 83.38 & 88.12 & 56.45 & 128.09 & 150.12 & 117.74 \\
TokenHMR~\cite{tokenhmr}     & 76.01 & 74.70 & 49.94 & 136.52 & 146.12 & 91.00 \\
AJAHR (Ours)             & \textbf{73.42} & \textbf{73.19} & \textbf{49.42} & 116.42 & \textbf{129.25} & \textbf{77.18} \\
\hline
\end{tabular}
}
\caption{\textbf{Comparison of Human Mesh Recovery on Amputee Data.} AJAHR is trained using the cross attention method and partially fine-tuning. The A3D evaluation was conducted using the A3D test dataset.}
\label{tab:amputation_table}
\end{table}


==> table/NON_AMPUTATION_DATASET_TABLE.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|ccc|ccc}
% \hline
% \multirow{2}{*}{Method} & \multicolumn{3}{c|}{EMDB~\cite{emdb}} & \multicolumn{3}{c}{3DPW~\cite{3dpw}} \\
% \cline{2-7}
%                         & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$
%                         & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
% \hline
% HMR2.0~\cite{4dhumans}       & 141.41 & 117.66 & 75.89 & 95.29 & 81.64 & 53.95 \\
% BEDLAM-CLIFF~\cite{bedlam, cliff} & 129.00 & 97.88  & 62.40 & 99.32 & 76.45 & 51.21 \\
% TokenHMR~\cite{tokenhmr}    & 113.26 & 93.77  & 58.98 & \textbf{90.23} & 72.87 & 47.17 \\
% AJAHR (Ours)             & \textbf{112.83} & \textbf{91.74} & \textbf{58.62} & 95.26 & \textbf{71.77} & \textbf{44.94} \\
% \hline
% \end{tabular}
% }
% \caption{\textbf{Comparison of Human Mesh Recovery on Non Amputee Data.} The evaluations for EMDB and 3DPW were conducted using their respective test datasets.}
% \label{tab:nonamputation_table}
% \end{table}


==> table/ablation.tex <==
\usepackage{graphicx} % 문서의 프리앰블에 추가

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{ % 컬럼 너비에 맞게 축소
\begin{tabular}{lccclllllllll}
\hline
\multirow{2}{*}{Method} &                            & EMDB~\cite{emdb}                      &                           &       & 3DPW~\cite{3dpw}  &          &       & AJAHR &          &        & ITW-amputee    &          \\ \cline{2-13} 
                        & MVE                        & MPJPE                     & PA-MPJPE                  & MVE   & MPJPE & PA-MPJPE & PVE   & MPJPE & PA-MPJPE & PVE    & MPJPE  & PA-MPJPE \\ \hline
AJAHR$\sim$             & 114.53                     & 94.37                     & 58.68                     & 97.16 & 72.68 & 46.00    & 74.98 & 74.45 & 48.8     & 121.62 & 133.73 & 77.94    \\
AJAHR*                  & \multicolumn{1}{l}{112.99} & \multicolumn{1}{l}{92.05} & \multicolumn{1}{l}{58.84} & 95.73 & 71.33 & 47.72    & 73.98 & 74.30 & 49.71    & 122.34 & 132.95 & 81.23    \\
AJAHR + CA              & \multicolumn{1}{l}{116.78} & \multicolumn{1}{l}{95.84} & \multicolumn{1}{l}{57.29} & 98.66 & 72.01 & 44.95    & 75.99 & 73.29 & 49.54    & 126.46 & 139.05 & 83.88    \\
AJAHR* + CA (Ours)      & 112.83                     & 91.74                     & 58.62                     & 95.26 & 71.77 & 44.94    & 73.42 & 73.19 & 49.42    & 116.42 & 129.25 & 77.18    \\ \hline
\end{tabular}
}
\end{table}


==> table/ablation_ajahr_nobpacnet.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3} 
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|ccc|ccc|ccc|ccc}
\hline
\textbf{Full} & \textbf{Partially} & \textbf{Cross} &
\multicolumn{3}{c|}{\textbf{EMDB}~\cite{emdb}} &
\multicolumn{3}{c|}{\textbf{3DPW}~\cite{3dpw}} &
\multicolumn{3}{c|}{\textbf{A3D}} &
\multicolumn{3}{c}{\textbf{ITW-amputee}} \\
\textbf{Fine Tuning} & \textbf{Fine Tuning} & \textbf{Attention} &
MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ &
MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ &
MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ &
MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
\hline
\checkmark  &             &             & 114.53 & 94.37 & 58.68 & 97.16 & 72.68 & 46.00 & 74.98 & 74.45 & \textbf{48.80} & 121.62 & 133.73 & 77.94 \\
            & \checkmark  &             & 112.99 & 92.05 & 58.84 & 95.73 & \textbf{71.33} & 47.72 & 73.98 & 74.30 & 49.71 & 122.34 & 132.95 & 81.23 \\
\checkmark  &             & \checkmark  & 116.78 & 95.84 & \textbf{57.29} & 98.66 & 72.01 & 44.95 & 75.99 & 73.29 & 49.54 & 126.46 & 139.05 & 83.88 \\
            & \checkmark  & \checkmark  & \textbf{112.83} & \textbf{91.74} & 58.62 & \textbf{95.26} & 71.77 & \textbf{44.94} & \textbf{73.42} & \textbf{73.19} & 49.42 & \textbf{116.42} & \textbf{129.25} & \textbf{77.18} \\
\hline
\end{tabular}
}
\vspace{1mm}
\caption{\textbf{Comparison of AJAHR Tuning Methods and the Presence of Cross Attention.} 
In \textit{Partially Fine-Tuning}, the main parameters of AJAHR are frozen, and only a limited subset of trainable parameters within each module is selectively updated. In contrast, \textit{Full Fine-Tuning} updates all parameters of AJAHR during training.}
\label{tab:ablation_ajahr_nobpac}
\end{table*}


==> table/ablation_classifier.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3} 
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc|ccc|ccc|ccc|ccc}
\hline
\textbf{Full}         & \textbf{Partially}   & \textbf{Cross}     & \textbf{Use}        & \multicolumn{3}{c|}{\textbf{EMDB}~\cite{emdb}}        & \multicolumn{3}{c|}{\textbf{3DPW}~\cite{3dpw}}         & \multicolumn{3}{c|}{\textbf{A3D}}         & \multicolumn{3}{c}{\textbf{ITW-amputee}}     \\
\textbf{Fine tuning}  & \textbf{Fine tuning} & \textbf{Attention} & \textbf{Classifier} & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ & PVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ & PVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
\hline
\checkmark            &                      &                    & \checkmark          & \textbf{113.42} & 97.33             & 59.87                & 97.98            & 73.68             & 47.76                & 89.34           & 89.96             & 69.87                & 143.49          & 154.83            & 85.17 \\
            & \checkmark           &                    & \checkmark          & 113.93          & 94.12             & 58.87                & 98.51            & 73.88             & 48.90                & 89.12           & 88.12             & 68.17                & 145.01          & 153.17            & 90.12 \\
\checkmark            &                      & \checkmark         & \checkmark          & 115.65          & 97.98             & 59.08                & 99.34            & 72.23             & 45.16                & 88.51           & 88.32             & 68.19                & 148.28          & 157.51            & 93.11 \\
            & \checkmark           & \checkmark         & \checkmark          & 114.52          & \textbf{93.73}    & \textbf{58.01}       & \textbf{97.02}   & \textbf{71.97}    & \textbf{44.98}       & \textbf{87.11}  & \textbf{87.91}    & \textbf{68.01}       & \textbf{139.64} & \textbf{143.74}   & \textbf{84.91} \\
\hline
\end{tabular}
}
\caption{\textbf{Comparison using the reconstructed mesh after BPAC's amputation inference.} After BPAC infers the amputation status, the corresponding label is used to force the inferred SMPL body pose parameters to zero. The evaluation is then conducted using 3D keypoints obtained from the reconstructed mesh.}
\label{tab:ablation_classifier_quant}
\end{table*}


==> table/ablation_tokenizer.tex <==
\begin{table*}[t]%\label{tab:pftorfft}
\centering
\renewcommand{\arraystretch}{1.3} 
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
\hline
Partially   & Cross     &                 & EMDB           &                &                & 3DPW           &                &                & A3D          &               &                 & ITW-amputee     &                \\ \cline{3-14} 
Fine Tuning & Attention & MVE             & MPJPE          & PA-MPJPE       & MVE            & MPJPE          & PA-MPJPE       & MVE            & MPJPE          & PA-MPJPE      & MVE             & MPJPE           & PA-MPJPE       \\ \hline
            &           & 114.53          & 94.37          & 58.68          & 97.16          & 72.68          & 46.00          & 74.98          & 74.45          & \textbf{48.8} & 121.62          & 133.73          & 77.94          \\
    \checkmark        &           & 112.99          & 92.05          & 58.84          & 95.73          & \textbf{71.33} & 47.72          & 73.98          & 74.30          & 49.71         & 122.34          & 132.95          & 81.23          \\
            &     \checkmark      & 116.78          & 95.84          & \textbf{57.29} & 98.66          & 72.01          & 44.95          & 75.99          & 73.29          & 49.54         & 126.46          & 139.05          & 83.88          \\
     \checkmark       &    \checkmark       & \textbf{112.83} & \textbf{91.74} & 58.62          & \textbf{95.26} & 71.77          & \textbf{44.94} & \textbf{73.42} & \textbf{73.19} & 49.42         & \textbf{116.42} & \textbf{129.25} & \textbf{77.18} \\ 
\end{tabular}}
\hline
\caption{\textbf{Comparison of AJAHR Tuning Methods and the Presence of Cross Attention.} Partially Fine-Tuning method freezes the AJAHR parameters while selectively updating a limited set of trainable parameters within each module. In contrast, Full Fine-Tuning updates all parameters of AJAHR during training.}
\label{tab:ablation_ajahr_main_quant}
\end{table*}


==> table/classifier.tex <==
\begin{table}[t]
\centering
\fontsize{6}{9.6}\selectfont
\resizebox{\columnwidth}{!}{ % 컬럼 너비에 맞게 축소
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{\textbf{Category}} & \multicolumn{2}{c}{3DPW-TEST~\cite{3dpw}} & \multicolumn{2}{c}{AJAHR-TEST} \\ \cline{2-5} 
                                   & Accuracy      & F1 Score      & Accuracy       & F1 Score      \\ \hline
Left Arm                           & 98.58         & 99.23         & 85.97          & 87.13         \\
Left Leg                           & 94.41         & 96.44         & 87.36          & 89.34         \\
Right Arm                          & 96.74         & 98.10         & 96.8           & 97.08         \\
Right Leg                          & 97.92         & 98.80         & 95.94          & 96.29         \\ \hline
\end{tabular}}
\end{table}


==> table/generation_quality.tex <==

\caption{EMDB를 이용해서 만든 엄선한 데이터셋인 AOdataset과 인터넷에서 긁어온 Paralympic선수들의 데이터셋인 ParaDatset(한다면 만들어야함.)  이 둘을 섞은 데이터셋에 대해 각각 MGDNet의 이미지 생성능력을 FID score로 나타낸다.}
\label{tab:generation_quality}
\begin{tabular}{@{}cll@{}}
\toprule
\multicolumn{1}{l}{Model Name} & Dataset                                                           & FID Score \\ \midrule
\multirow{MGDNet}        & AODataset                                                         & 20        \\
                               & ParaDataset                                                       & 15        \\
                               & \begin{tabular}[c]{@{}l@{}}AODataset\\ + ParaDataset\end{tabular} & 17       
\end{tabular}


==> table/indexes.tex <==
\caption{Body Parts and their Corresponding Indices}
\label{tab:part_index}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Index} & \textbf{Body Parts Name} \\ \hline
0             & Ri\input{chapter/3_METHODS}ght wrist               \\ \hline
1             & Right elbow            \\ \hline
2             & Right shoulder                \\ \hline
3             & Left wrist                \\ \hline
4             & Left elbow             \\ \hline
5             & Left shoulder                 \\ \hline
6             & Left ankle                \\ \hline
7             & Left knee                 \\ \hline
8             & Left hip              \\ \hline
9             & Right ankle               \\ \hline
10            & Right knee                \\ \hline
11            & Right hip                    \\ \hline
\end{tabular}


==> table/main_table.tex <==
% \begin{table}[t]  % 첫 번째 테이블 (Amputation)
%     \centering
%     \caption{Comparison of Human Mesh Recovery on Amputee Data.}
%     \label{tab:amputation_table}
%     \input{ICCV2025-Author-Kit-Feb/table/AMPUTATION_DATASET_TABLE}
% \end{table}

% \vspace{15pt} % 테이블 간격 추가

% \begin{table}[t]  % 두 번째 테이블 (Non-Amputation)
%     \centering
%     \caption{Comparison of Human Mesh Recovery on Non-Amputee Data.}
%     \label{tab:non_amputation_table}
%     \input{ICCV2025-Author-Kit-Feb/table/NON_AMPUTATION_DATASET_TABLE}
% \end{table}


==> table/perform_comparison_eachdatastyle.tex <==
\begin{table*}[t]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{A3D} & \multicolumn{3}{c}{ITW-amputee} \\ 
\cline{2-7}
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
\hline
HMR2.0~\cite{4dhumans}       & 89.35 & 96.75 & 86.14 & \textbf{110.33} & 154.43 & 121.83 \\
BEDLAM-CLIFF~\cite{bedlam, cliff} & 83.38 & 88.12 & 56.45 & 128.09 & 150.12 & 117.74 \\
TokenHMR~\cite{tokenhmr}     & 76.01 & 74.70 & 49.94 & 136.52 & 146.12 & 91.00 \\
AJAHR (Ours)             & \textbf{73.42} & \textbf{73.19} & \textbf{49.42} & 116.42 & \textbf{129.25} & \textbf{77.18} \\
\hline
\end{tabular}
}
\caption{\textbf{Comparison of Human Mesh Recovery on Amputee Data.}}
\label{tab:amputation_table}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{EMDB~\cite{emdb}} & \multicolumn{3}{c}{3DPW~\cite{3dpw}} \\
\cline{2-7}
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$
                        & MVE$\downarrow$ & MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ \\
\hline
HMR2.0~\cite{4dhumans}       & 141.41 & 117.66 & 75.89 & 95.29 & 81.64 & 53.95 \\
BEDLAM-CLIFF~\cite{bedlam, cliff} & 129.00 & 97.88  & 62.40 & 99.32 & 76.45 & 51.21 \\
TokenHMR~\cite{tokenhmr}    & 113.26 & 93.77  & 58.98 & \textbf{90.23} & 72.87 & 47.17 \\
AJAHR (Ours)             & \textbf{112.83} & \textbf{91.74} & \textbf{58.62} & 95.26 & \textbf{71.77} & \textbf{44.94} \\
\hline
\end{tabular}
}
\caption{\textbf{Comparison of Human Mesh Recovery on Non-Amputee Data.}}
\label{tab:nonamputation_table}
\end{minipage}
\end{table*}


==> table/quantitative.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|ccclllllllll} 
\toprule
\multirow{2}{*}{Method}           &        & EMDB   & \multicolumn{1}{c|}{}         &       & 3DPW  & \multicolumn{1}{l|}{}         &       & AJAHR & \multicolumn{1}{l|}{}         &        & a2d    &           \\ 
\cline{2-13}
                                  & MVE    & MPJPE  & \multicolumn{1}{c|}{PA-MPJPE} & MVE   & MPJPE & \multicolumn{1}{l|}{PA-MPJPE} & PVE   & MPJPE & \multicolumn{1}{l|}{PA-MPJPE} & PVE    & MPJPE  & PA-MPJPE  \\ 
\hline
HMR2.0                            & 141.41 & 117.66 & 75.89                         & 95.29 & 81.64 & 53.95                         & 89.35 & 96.75 & 86.14                         & 110.33 & 154.43 & 121.83    \\
BEDLAM-CLIFF                      &        &        &                               &       &       &                               &       &       &                               &        &        &           \\
TokenHMR                          & 113.26 & 93.77  & 58.98                         & 90.23 & 72.87 & 47.17                         & 76.01 & 74.70 & 49.94                         & 136.52 & 146.12 & 91.00     \\
AJAHR (Full Fine Tuning)          & 114.53 & 94.37  & 58.68                         & 97.16 & 72.68 & 46.00                         & 74.98 & 74.45 & 48.8                          & 121.62 & 133.73 & 77.94     \\
AJAHR (Partially Fine-Tuning)     & 112.99 & 92.05  & 58.84                         & 95.73 & 71.33 & 47.72                         & 73.98 & 74.30 & 49.71                         & 122.34 & 132.95 & 81.23     \\
AJAHR + CA (Full Fine Tuning)     & 116.78 & 95.84  & 57.29                         & 98.66 & 72.01 & 44.95                         & 75.99 & 73.29 & 49.54                         & 126.46 & 139.05 & 83.88     \\
AJAHR + CA(Partially Fine-Tuning) & 112.83 & 91.74  & 58.62                         & 95.26 & 71.77 & 44.94                         & 73.42 & 73.19 & 49.42                         & 116.42 & 129.25 & 77.18     \\
\bottomrule
\end{tabular}
\end{table}


==> table/rebuttal/implementation_detail_kor.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{|l|p{6.2cm}|p{6.2cm}|}
\hline
\textbf{항목} & \textbf{AJAHR} & \textbf{AJAHR-Tokenizer} \\
\hline
학습 대상 모듈 & ViTPose 마지막 4블록, Patch Embedding, Pose Embedding, Transformer Decoder 마지막 2블록, Bridge MLP & VQ-VAE 전체 (인코더, 디코더, 코드북 포함) \\
\hline
학습 방식 & 부분 미세 조정 (Partially Fine-Tuning) & 전체 학습 (Full Training) \\
\hline
학습 데이터셋 & A3D, 비결손 정상인 벤치마크 & AMASS, MOYO, A3D \\
\hline
배치 사이즈 & 64 × 2 (병렬 학습) & 256 \\
\hline
최적화 알고리즘 & AdamW & AdamW \\
\hline
Weight Decay & 1e-−4 & 1e-−5 \\
\hline
Learning Rate & 5e−-6 & 2e−-4 \\
\hline
Gamma (감마) & - & 5e−2 \\
\hline
총 학습 반복 수 & 150,000회 & 200,000회 \\
\hline
SMPL Variant & SMPL & SMPLH \\

\hline
코드북 차원 수 & - & 256 \\
\hline
코드 개수 & - & 2048 \\
\hline
토큰 개수 & - & 160 \\
\hline
\end{tabular}
\caption{AJAHR와 AJAHR-Tokenizer의 학습 설정 비교}
\label{tab:training_settings}
\end{table*}


==> table/rebuttal/rebuttal_3DOH50K.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{l|lllll}
\hline
Dataset & \multicolumn{5}{c}{3DOH50K[C3]}                                                                                                          \\ \hline
Metric & \multicolumn{1}{l|}{PA-MPJPE} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & F1    \\ \hline
Ours   & \multicolumn{1}{l|}{88.19}    & \multicolumn{1}{l|}{0.956}    & \multicolumn{1}{l|}{0.956}     & \multicolumn{1}{l|}{1.0}    & 0.977 \\ \hline
\end{tabular}
}
\vspace{-2mm}
\caption{Evaluation results on 3DOH50K[C3] using the AJAHR model.}
\label{tab:occ_3doh50k}
\vspace{-2mm}
\end{table}

==> table/rebuttal/rebuttal_3doh50k_and_A3D.tex <==
\begin{table}[t]
\centering
\small % 혹은 \scriptsize, \tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|cccc}
\hline
Dataset & \multicolumn{4}{c|}{A3D(amputation)}                                                                             & \multicolumn{4}{c}{3DOH50K\footnotemark[4](occlusion)}                                                                 \\ \hline
Metric  & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & F1    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & F1    \\ \hline
Ours    & \multicolumn{1}{c|}{0.881}    & \multicolumn{1}{c|}{0.756}     & \multicolumn{1}{c|}{0.922}  & 0.820 & \multicolumn{1}{c|}{0.956}    & \multicolumn{1}{c|}{0.956}     & \multicolumn{1}{c|}{1.0}    & 0.977 \\ \hline
\end{tabular}}
\vspace{-4mm}
\caption{\textbf{BPAC-Net evaluation on A3D and 3DOH50K\cite{3doh50k} datasets.} Average classification performance across all classifier heads, computed from confusion matrices.}
\label{tab:occ_3doh50k}
\vspace{-3mm}
\end{table}


% CCI~\tablefootnote{A Guide for Users of the Canadian Classification of Health Interventions (CCI)..., CIHI2015}
% 3DOH50K~\tablefootnote{Object-occluded human shape and pose estimation from a single color image..., CVPR2020}
% LPIPS~\tablefootnote{The unreasonable effectiveness of deep features as a perceptual metric..., CVPR2018}

\footnotetext[4]{Object-occluded human shape and pose estimation from..., CVPR2020}


==> table/rebuttal/rebuttal_a3d_bpac_metric.tex <==
\begin{table}[t]
\begin{tabular}{c|cccc|cccc}
\hline
Dataset & \multicolumn{4}{c|}{A3D}                                                                             & \multicolumn{4}{c}{3DOH50K {[}C3{]}}                                                                 \\ \hline
Metric  & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & F1    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & F1    \\ \hline
Ours    & \multicolumn{1}{c|}{0.881}    & \multicolumn{1}{c|}{0.756}     & \multicolumn{1}{c|}{0.922}  & 0.820 & \multicolumn{1}{c|}{0.956}    & \multicolumn{1}{c|}{0.956}     & \multicolumn{1}{c|}{1.0}    & 0.977 \\ \hline
\end{tabular}
\end{table}

==> table/rebuttal/rebuttal_baseline.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
Dataset &
  \multicolumn{3}{c|}{EMDB(Real)} &
  \multicolumn{3}{c|}{3DPW(Real)} &
  \multicolumn{3}{c|}{A3D(Synthetic)} &
  \multicolumn{3}{c}{ITW-amputee(Real)} \\ \hline
Metric &
  \multicolumn{1}{c|}{MVE\,$\downarrow$} &
  \multicolumn{1}{c|}{MPJPE\,$\downarrow$} &
  PA-MPJPE\,$\downarrow$ &
  \multicolumn{1}{c|}{MVE\,$\downarrow$} &
  \multicolumn{1}{c|}{MPJPE\,$\downarrow$} &
  PA-MPJPE\,$\downarrow$ &
  \multicolumn{1}{c|}{MVE\,$\downarrow$} &
  \multicolumn{1}{c|}{MPJPE\,$\downarrow$} &
  PA-MPJPE\,$\downarrow$ &
  \multicolumn{1}{c|}{MVE\,$\downarrow$} &
  \multicolumn{1}{c|}{MPJPE\,$\downarrow$} &
  PA-MPJPE\,$\downarrow$ \\ \hline
4DHumans] &
  \multicolumn{1}{c|}{149.31} &
  \multicolumn{1}{c|}{125.69} &
  80.74 &
  \multicolumn{1}{c|}{100.21} &
  \multicolumn{1}{c|}{89.74} &
  56.91 &
  \multicolumn{1}{c|}{104.72} &
  \multicolumn{1}{c|}{104.75} &
  94.32 &
  \multicolumn{1}{c|}{134.71} &
  \multicolumn{1}{c|}{176.46} &
  132.27 \\ \hline
BEDLAM-CLIFF &
  \multicolumn{1}{c|}{133.75} &
  \multicolumn{1}{c|}{100.29} &
  73.24 &
  \multicolumn{1}{c|}{103.98} &
  \multicolumn{1}{c|}{83.21} &
  54.28 &
  \multicolumn{1}{c|}{92.77} &
  \multicolumn{1}{c|}{96.48} &
  75.87 &
  \multicolumn{1}{c|}{147.51} &
  \multicolumn{1}{c|}{166.07} &
  126.90 \\ \hline
Ours &
  \multicolumn{1}{c|}{\textbf{114.52}} &
  \multicolumn{1}{c|}{\textbf{93.73}} &
  \textbf{58.01} &
  \multicolumn{1}{c|}{\textbf{97.02}} &
  \multicolumn{1}{c|}{\textbf{71.97}} &
  \textbf{44.98} &
  \multicolumn{1}{c|}{\textbf{87.11}} &
  \multicolumn{1}{c|}{\textbf{87.91}} &
  \textbf{68.01} &
  \multicolumn{1}{c|}{\textbf{139.64}} &
  \multicolumn{1}{c|}{\textbf{143.74}} &
  \textbf{84.91} \\ \hline
\end{tabular}
}
\vspace{-4mm}
\caption{Simple baselines with BPAC-Net Vs. AJAHR.}
\label{tab:baseline}
\vspace{-8mm}
\end{table}

% 4DHumans~\tablefootnote{Humans in 4D: Reconstructing and tracking humans..., ICCV2023}
% BEDLAM~\tablefootnote{BEDLAM:A Synthetic Dataset of Bodies..., CVPR2023}

% \footnotetext[7]{Humans in 4D: Reconstructing and tracking humans..., ICCV2023}
% \footnotetext[8]{BEDLAM:A Synthetic Dataset of Bodies..., CVPR2023}


==> table/rebuttal/rebuttal_classifier_keypoint_or_heatmap.tex <==
% \begin{table}[t]
% \centering
% \small % 혹은 \scriptsize, \tiny
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% BPAC &  & EMDB  && & 3DPW &  &  & AJAHR &   & & ITW-amputee &  \\ \hline
% Type          & MVE    & MPJPE  & PA-MPJPE       & MVE    & MPJPE          & PA-MPJPE & MVE   & MPJPE & PA-MPJPE       & MVE    & MPJPE  & PA-MPJPE \\ \hline
% Image only    & 121.81 & 100.98 & 70.21          & 103.71 & 77.09          & 49.54    & 95.88 & 93.12 & 75.44 & 145.21 & 150.55 & 92.71    \\ \hline
% Keypoint only & 118.21 & 96.12  & 61.71          & 100.87 & 74.87 & 46.91    & 90.12 & 89.21 & 70.77          & 141.64 & 146.21 & 87.88    \\ \hline
% Ours          & 114.52 & 93.73  & 58.01 & 97.02  & 71.97          & 44.98    & 87.11 & 87.91 & 68.01          & 139.64 & 143.74 & 84.91    \\ \hline
% \end{tabular}
% }
% \caption{dddddddddd}
% \label{tab:bpac-abl}
% \end{table}
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
\textbf{Dataset} & \multicolumn{3}{c|}{EMDB\footnotemark[1](Real)}                                                          & \multicolumn{3}{c|}{3DPW(Real)}                                                         & \multicolumn{3}{c|}{A3D(Synthetic)}                                                        & \multicolumn{3}{c}{ITW-amputee(Real)}                                                     \\ \hline
Metric           & \multicolumn{1}{c|}{MVE}             & \multicolumn{1}{c|}{MPJPE}          & PA-MPJPE       & \multicolumn{1}{c|}{MVE}            & \multicolumn{1}{c|}{MPJPE}          & PA-MPJPE       & \multicolumn{1}{c|}{MVE}            & \multicolumn{1}{c|}{MPJPE}          & PA-MPJPE       & \multicolumn{1}{c|}{MVE}             & \multicolumn{1}{c|}{MPJPE}           & PA-MPJPE       \\ \hline
Image only       & \multicolumn{1}{c|}{131.81}          & \multicolumn{1}{c|}{109.98}         & 74.21          & \multicolumn{1}{c|}{113.71}         & \multicolumn{1}{c|}{87.09}          & 59.54          & \multicolumn{1}{c|}{105.88}         & \multicolumn{1}{c|}{103.12}         & 85.44          & \multicolumn{1}{c|}{152.21}          & \multicolumn{1}{c|}{154.55}          & 92.71          \\ \hline
Keypoint only    & \multicolumn{1}{c|}{118.21}          & \multicolumn{1}{c|}{96.12}          & 61.71          & \multicolumn{1}{c|}{100.87}         & \multicolumn{1}{c|}{74.87}          & 46.91          & \multicolumn{1}{c|}{90.12}          & \multicolumn{1}{c|}{89.21}          & 70.77          & \multicolumn{1}{c|}{141.64}          & \multicolumn{1}{c|}{146.21}          & 87.88          \\ \hline
Ours             & \multicolumn{1}{c|}{\textbf{114.52}} & \multicolumn{1}{c|}{\textbf{93.73}} & \textbf{58.01} & \multicolumn{1}{c|}{\textbf{97.02}} & \multicolumn{1}{c|}{\textbf{71.97}} & \textbf{44.98} & \multicolumn{1}{c|}{\textbf{87.11}} & \multicolumn{1}{c|}{\textbf{87.91}} & \textbf{68.01} & \multicolumn{1}{c|}{\textbf{139.64}} & \multicolumn{1}{c|}{\textbf{143.74}} & \textbf{84.91} \\ \hline
\end{tabular}
}
\vspace{-4mm}
\caption{BPAC ablation study.}
\label{tab:bpac-abl}
\vspace{-4mm}
\end{table}

% EMDB~\tablefootnote{Emdb:The electromagnetic database of..., ICCV2023}
% 3DPW~\tablefootnote{3DPW:Recovering Accurate 3D Human Pose..., ECCV2018}
% \footnotetext[2]{EMDB: The Electromagnetic Database of..., ICCV 2023}
% \footnotetext[3]{3DPW: Recovering Accurate 3D Human Pose..., ECCV 2018}

==> table/rebuttal/rebuttal_lpips.tex <==
\begin{table}[t]
\centering
\small % 혹은 \scriptsize, \tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
Dataset     & A3D(MPII) & A3D(MSCOCO) & A3D(H3.6M) & 
Avg. \\ \hline
LPIPS~\cite{lpips},$\downarrow$ & 0.0735        & 0.0421          & 0.16186        & 0.155         \\ \hline
\end{tabular}
}
\caption{LPIPS scores for A3D across datasets.}
\label{tab:lpips}
\end{table}


==> table/rebuttal/rebuttal_noise.tex <==
\begin{table}[t]
\centering
\small % 혹은 \scriptsize, \tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
Noise & \multicolumn{3}{c|}{EMDB(Real)}                                                                   & \multicolumn{3}{c|}{3DPW(Real)}                                                                  & \multicolumn{3}{c|}{AJAHR(Synthetic)}                                                                 & \multicolumn{3}{c}{ITW-amputee(Real)}                                                              \\ \cline{2-13} 
Ratio & \multicolumn{1}{c|}{MVE\,$\downarrow$}             & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{MVE\,$\downarrow$}            & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{PVE\,$\downarrow$}            & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{PVE\,$\downarrow$}             & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}           & PA-MPJPE\,$\downarrow$       \\ \hline
Ours  & \multicolumn{1}{c|}{\textbf{112.83}} & \multicolumn{1}{c|}{\textbf{91.74}} & \textbf{58.62} & \multicolumn{1}{c|}{\textbf{95.26}} & \multicolumn{1}{c|}{\textbf{71.77}} & \textbf{44.94} & \multicolumn{1}{c|}{\textbf{73.42}} & \multicolumn{1}{c|}{\textbf{73.19}} & \textbf{49.42} & \multicolumn{1}{c|}{\textbf{116.42}} & \multicolumn{1}{c|}{\textbf{129.25}} & \textbf{77.18} \\ \hline
25\%  & \multicolumn{1}{c|}{113.01}          & \multicolumn{1}{c|}{92.02}          & 58.88          & \multicolumn{1}{c|}{95.76}          & \multicolumn{1}{c|}{72.08}          & 45.08          & \multicolumn{1}{c|}{73.98}          & \multicolumn{1}{c|}{73.87}          & 50.11          & \multicolumn{1}{c|}{118.41}          & \multicolumn{1}{c|}{131.37}          & 79.21          \\ \hline
50\%  & \multicolumn{1}{c|}{114.31}          & \multicolumn{1}{c|}{93.12}          & 59.22          & \multicolumn{1}{c|}{96.43}          & \multicolumn{1}{c|}{72.77}          & 45.87          & \multicolumn{1}{c|}{74.76}          & \multicolumn{1}{c|}{74.21}          & 50.89          & \multicolumn{1}{c|}{121.21}          & \multicolumn{1}{c|}{134.91}          & 80.01          \\ \hline
75\%  & \multicolumn{1}{c|}{115.07}          & \multicolumn{1}{c|}{93.78}          & 59.31          & \multicolumn{1}{c|}{96.91}          & \multicolumn{1}{c|}{73.31}          & 46.88          & \multicolumn{1}{c|}{75.12}          & \multicolumn{1}{c|}{74.59}          & 51.78          & \multicolumn{1}{c|}{123.95}          & \multicolumn{1}{c|}{135.34}          & 82.51          \\ \hline
100\% & \multicolumn{1}{c|}{116.71}          & \multicolumn{1}{c|}{94.22}          & 59.97          & \multicolumn{1}{c|}{98.03}          & \multicolumn{1}{c|}{74.64}          & 48.31          & \multicolumn{1}{c|}{76.87}          & \multicolumn{1}{c|}{76.12}          & 52.04          & \multicolumn{1}{c|}{127.77}          & \multicolumn{1}{c|}{137.78}          & 85.22          \\ \hline
\end{tabular}
}
\vspace{-4mm}
\caption{Effect of keypoint noise on evaluation.}
\label{tab:noise_ratio_results}
\vspace{-4mm}
\end{table}



==> table/rebuttal/rebuttal_tokenizer.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{cc|cccccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Method}}                                                         & \multicolumn{2}{c}{AJAHR}     & \multicolumn{2}{c}{AMASS$\sim$\textbackslash{}cite\{AMASS\}} & \multicolumn{2}{c}{MOYO$\sim$\textbackslash{}cite\{moyo\}} \\ \cline{3-8} 
\multicolumn{2}{c|}{}                                                                                & MPJPE         & MVE           & MPJPE                         & MVE                          & MPJPE                       & MVE                          \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Code\\ Book\end{tabular}}} & 128x2048 & 1.72          & 8.05          & 2.24                          & 8.62                         & 7.49                        & 16.5                         \\
\multicolumn{1}{c|}{}                                                                     & 256x1024 & 1.92          & 8.50          & 2.50                          & 8.80                         & 7.15                        & 16.18                        \\
\multicolumn{1}{c|}{}                                                                     & 256x2048 & \textbf{1.56} & \textbf{8.01} & \textbf{1.90}                 & \textbf{8.08}                & \textbf{5.52}               & \textbf{13.47}               \\ \hline
\multicolumn{1}{c|}{Tokens}                                                               & 20       & 5.51          & 12.6          & 7.62                          & 15.0                         & 23.10                       & 38.87                        \\
\multicolumn{1}{c|}{}                                                                     & 40       & 3.49          & 9.76          & 4.51                          & 10.67                        & 14.50                       & 26.04                        \\
\multicolumn{1}{c|}{}                                                                     & 80       & 2.39          & 8.56          & 3.07                          & 8.97                         & 10.05                       & 19.44                        \\
\multicolumn{1}{c|}{}                                                                     & 160      & \textbf{2.07} & \textbf{8.38} & 2.74                          & \textbf{8.67}                & \textbf{6.68}               & \textbf{14.6}                \\
\multicolumn{1}{c|}{}                                                                     & 640      & 2.59          & 9.03          & \textbf{2.60}                 & 9.03                         & 8.02                        & 16.6                         \\ \cline{2-8} 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \footnotetext[5]{AMASS: Archive of motion capture as surface shapes..., ICCV2019}
% \footnotetext[6]{MOYO:A dataset containing complex yoga poses..., CVPR2023}

==> table/rebuttal/rebuttal_tokenizer_switching_single_dual.tex <==
\begin{table}[t]
\centering
\small % 혹은 \scriptsize, \tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
Dataset             &                                      & EMDB(Real)                                &                &                                     & 3DPW(Real)                                &                &                                     & AJAHR(Synthetic)                               &                &                                      & ITW-amputee(Real)                          &                \\ \hline
Metric              & \multicolumn{1}{c|}{MVE\,$\downarrow$}             & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{MVE\,$\downarrow$}            & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{MVE\,$\downarrow$}            & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}          & PA-MPJPE\,$\downarrow$       & \multicolumn{1}{c|}{MVE\,$\downarrow$}             & \multicolumn{1}{c|}{MPJPE\,$\downarrow$}           & PA-MPJPE\,$\downarrow$       \\ \hline
Amputation Only     & \multicolumn{1}{c|}{115.70}          & \multicolumn{1}{c|}{93.75}          & 59.08          & \multicolumn{1}{c|}{96.32}          & \multicolumn{1}{c|}{72.76}          & 45.92          & \multicolumn{1}{c|}{74.71}          & \multicolumn{1}{c|}{74.51}          & 49.93 & \multicolumn{1}{c|}{118.09}          & \multicolumn{1}{c|}{131.12}          & 78.08          \\ \hline
Non Amputation Only & \multicolumn{1}{c|}{113.09}          & \multicolumn{1}{c|}{92.07}          & \textbf{57.97} & \multicolumn{1}{c|}{95.34}          & \multicolumn{1}{c|}{\textbf{72.02}} & 45.02          & \multicolumn{1}{c|}{76.01}          & \multicolumn{1}{c|}{76.31}          & 50.99          & \multicolumn{1}{c|}{120.81}          & \multicolumn{1}{c|}{134.71}          & 81.82          \\ \hline
Ours                & \multicolumn{1}{c|}{\textbf{112.83}} & \multicolumn{1}{c|}{\textbf{91.74}} & 58.62          & \multicolumn{1}{c|}{\textbf{95.26}} & \multicolumn{1}{c|}{\textbf{71.77}} & \textbf{44.94} & \multicolumn{1}{c|}{\textbf{73.42}} & \multicolumn{1}{c|}{\textbf{73.19}} & \textbf{49.42} & \multicolumn{1}{c|}{\textbf{116.42}} & \multicolumn{1}{c|}{\textbf{129.25}} & \textbf{77.18} \\ \hline
\end{tabular}
}
\vspace{-5mm}
\caption{Comparison of Single vs. Dual Tokenizer(Ours).}
\label{tab:single-tokenizer}
\vspace{-4mm}
\end{table}



==> table/tokenizer_ablations.tex <==
\begin{table*}[t]%\label{tab:pftorfft}
\centering
\renewcommand{\arraystretch}{1.3} 
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
\hline
Partially   & Cross     &                 & EMDB           &                &                & 3DPW           &                &                & A3D          &               &                 & ITW-amputee     &                \\ \cline{3-14} 
Fine Tuning & Attention & MVE             & MPJPE          & PA-MPJPE       & MVE            & MPJPE          & PA-MPJPE       & MVE            & MPJPE          & PA-MPJPE      & MVE             & MPJPE           & PA-MPJPE       \\ \hline
            &           & 114.53          & 94.37          & 58.68          & 97.16          & 72.68          & 46.00          & 74.98          & 74.45          & \textbf{48.8} & 121.62          & 133.73          & 77.94          \\
    \checkmark        &           & 112.99          & 92.05          & 58.84          & 95.73          & \textbf{71.33} & 47.72          & 73.98          & 74.30          & 49.71         & 122.34          & 132.95          & 81.23          \\
            &     \checkmark      & 116.78          & 95.84          & \textbf{57.29} & 98.66          & 72.01          & 44.95          & 75.99          & 73.29          & 49.54         & 126.46          & 139.05          & 83.88          \\
     \checkmark       &    \checkmark       & \textbf{112.83} & \textbf{91.74} & 58.62          & \textbf{95.26} & 71.77          & \textbf{44.94} & \textbf{73.42} & \textbf{73.19} & 49.42         & \textbf{116.42} & \textbf{129.25} & \textbf{77.18} \\ 
\end{tabular}}
\hline
\caption{\textbf{Comparison of AJAHR Tuning Methods and the Presence of Cross Attention.} Partially Fine-Tuning method freezes the AJAHR parameters while selectively updating a limited set of trainable parameters within each module. In contrast, Full Fine-Tuning updates all parameters of AJAHR during training.}
\label{tab:ablation_ajahr_main_quant}
\end{table*}

